On the Robustness and Scalability of Semidefinite Relaxation for Optimal Power Flow Problems

Semidefinite relaxation techniques have shown great promise for nonconvex optimal power flow problems. However, a number of independent numerical experiments have led to concerns about scalability and robustness of existing SDP solvers. To address these concerns, we investigate some numerical aspects of the problem and compare different state-of-the-art solvers. Our results demonstrate that semidefinite relaxations of large problem instances with on the order of 10,000 buses can be solved reliably and to reasonable accuracy within minutes. Furthermore, the semidefinite relaxation of a test case with 25,000 buses can be solved reliably within half an hour; the largest test case with 82,000 buses is solved within eight hours. We also compare the lower bound obtained via semidefinite relaxation to locally optimal solutions obtained with nonlinear optimization methods and calculate the optimality gap.

==> files/matpower_table.tex <==
\begin{sidewaystable}[htb]
%\normalsize
\centering
\caption{Cost, gap, and computation time for cases with more than 300 buses and without dispatchable loads from the MATPOWER library. Failures are reported as `M' (max.\ iterations), `I' (termination at infeasible point), and `N' (numerical error in solver). Computational times shown in \textcolor{red}{red} correspond to failures.}
\label{tab:cases_matpower}
\begin{tabular}{c|l|rrrr|r|dddd}
\toprule
&  & \multicolumn{4}{c|}{Cost} & \multicolumn{1}{c|}{Gap} & \multicolumn{4}{c}{Time (seconds)} \\
& Case & \multicolumn{1}{c}{IPOPT} & \multicolumn{1}{c}{KNITRO} & \multicolumn{1}{c}{MIPS} & \multicolumn{1}{c|}{MOSEK} &                     & \multicolumn{1}{c}{IPOPT} & \multicolumn{1}{c}{KNITRO} & \multicolumn{1}{c}{MIPS} & \multicolumn{1}{c}{MOSEK} \\
\hline
\multirow{24}{*}{\rotatebox[origin=c]{90}{MATPOWER}}
 & ACTIVSg500 & 7.258e+04 & 7.258e+04 & 7.258e+04 & 7.105e+04 & 2.1\% & 0.8 & 0.7 & 0.7 & 4.4\\
 & 1354pegase & 7.407e+04 & 7.407e+04 & 7.407e+04 & 7.406e+04 & 0.0\% & 1.9 & 2.0 & 2.6 & 9.3\\
 & 1888rte & M & 5.986e+04 & N & 5.960e+04 & 0.4\% & \dcolcolor{red} 3,\!264 & 31.6 & \dcolcolor{red} 1.1 & 14.8\\
 & 1951rte & 8.174e+04 & I & N & 8.174e+04 & 0.0\% & 20.6 & \dcolcolor{red} 61.8 & \dcolcolor{red} 1.4 & 17.6\\
 & ACTIVSg2000 & 1.228e+06 & 1.228e+06 & 1.228e+06 & 1.228e+06 & 0.0\% & 7.6 & 2.8 & 8.3 & 116\\
 & 2383wp & 1.869e+06 & 1.869e+06 & 1.869e+06 & 1.863e+06 & 0.3\% & 3.1 & 3.4 & 3.5 & 63.8\\
 & 2736sp & 1.308e+06 & 1.308e+06 & 1.308e+06 & 1.307e+06 & 0.1\% & 3.3 & 3.0 & 3.5 & 64.6\\
 & 2737sop & 7.776e+05 & 7.776e+05 & 7.776e+05 & 7.772e+05 & 0.1\% & 2.8 & 3.0 & 3.3 & 60.3\\
 & 2746wp & 1.632e+06 & 1.632e+06 & 1.632e+06 & 1.631e+06 & 0.0\% & 3.3 & 3.0 & 3.6 & 70.1\\
 & 2746wop & 1.208e+06 & 1.208e+06 & 1.208e+06 & 1.208e+06 & 0.0\% & 3.0 & 3.1 & 3.8 & 72.3\\
 & 2848rte & M & I & N & 5.301e+04 &  \textemdash  & \dcolcolor{red} 3,\!062 & \dcolcolor{red} 20.4 & \dcolcolor{red} 2.2 & 21.4\\
 & 2868rte & M & 7.979e+04 & N & 7.980e+04 & -0.0\% & \dcolcolor{red} 780 & 47.2 & \dcolcolor{red} 2.7 & 25.7\\
 & 2869pegase & 1.340e+05 & 1.340e+05 & 1.340e+05 & 1.340e+05 & 0.0\% & 3.3 & 3.3 & 5.2 & 25.9\\
 & 3012wp & 2.592e+06 & 2.592e+06 & 2.592e+06 & 2.588e+06 & 0.1\% & 4.8 & 4.8 & 5.5 & 112\\
 & 3120sp & 2.143e+06 & 2.143e+06 & 2.143e+06 & 2.141e+06 & 0.1\% & 5.1 & 4.3 & 6.2 & 122\\
 & 3375wp & 7.412e+06 & 7.412e+06 & 7.412e+06 & 7.408e+06 & 0.1\% & 8.5 & 4.6 & 8.4 & 97.6\\
 & 6468rte & 8.683e+04 & 8.683e+04 & N & 8.681e+04 & 0.0\% & 1,\!530 & 93.9 & \dcolcolor{red} 12.3 & 83.5\\
 & 6470rte & M & I & N & 9.834e+04 &  \textemdash  & \dcolcolor{red} 53.4 & \dcolcolor{red} 18.3 & \dcolcolor{red} 24.6 & 101\\
 & 6495rte & M & I & N & 1.061e+05 &  \textemdash  & \dcolcolor{red} 2,\!943 & \dcolcolor{red} 124 & \dcolcolor{red} 10.5 & 104\\
 & 6515rte & 1.098e+05 & 1.098e+05 & N & 1.097e+05 & 0.1\% & 1,\!060 & 108 & \dcolcolor{red} 12.4 & 106\\
 & 9241pegase & 3.159e+05 & 3.159e+05 & 3.159e+05 & 3.159e+05 & 0.0\% & 70.9 & 100 & 24.0 & 183\\
 & ACTIVSg10k & 2.486e+06 & I & N & 2.486e+06 & -0.0\% & 74.3 & \dcolcolor{red} 139 & \dcolcolor{red} 58.3 & 351\\
 & 13659pegase & M & 3.861e+05 & N & 3.861e+05 & -0.0\% & \dcolcolor{red} 125 & 171 & \dcolcolor{red} 4,\!925 & 145\\
 & ACTIVSg25k & 6.018e+06 & 6.018e+06 & N & 6.016e+06 & 0.0\% & 91.0 & 64.8 & \dcolcolor{red} 103 & 3,\!592\\
\bottomrule
\end{tabular}
\end{sidewaystable}

==> files/mediumLargeTable.tex <==
\begin{sidewaystable}[htb]
\normalsize
\centering
%\rotatebox[origin=c]{90}{
% \begin{minipage}[c]{\textheight}
\caption{Cost, gap, and computation time for cases with more than 300 buses and without dispatchable loads. Failures are reported as `M' (max.\ iterations), `I' (termination at infeasible point), and `N' (numerical error in solver). Computational times shown in \textcolor{red}{red} correspond to failures.}
\label{tab:cases}
%\end{minipage} 
% }\begin{minipage}[c]{.85\textwidth}
\begin{tabular}{c|l|rrrr|r|dddd}
\toprule
&  & \multicolumn{4}{c|}{Cost} & \multicolumn{1}{c|}{Gap} & \multicolumn{4}{c}{Time (seconds)} \\
& Case & \multicolumn{1}{c}{IPOPT} & \multicolumn{1}{c}{KNITRO} & \multicolumn{1}{c}{MIPS} & \multicolumn{1}{c|}{MOSEK} &                     & \multicolumn{1}{c}{IPOPT} & \multicolumn{1}{c}{KNITRO} & \multicolumn{1}{c}{MIPS} & \multicolumn{1}{c}{MOSEK} \\
\hline
\multirow{24}{*}{\rotatebox[origin=c]{90}{MATPOWER}}
 & ACTIVSg500 & 7.258e+04 & 7.258e+04 & 7.258e+04 & 7.105e+04 & 2.1\% & 0.8 & 0.7 & 0.7 & 4.4\\
 & 1354pegase & 7.407e+04 & 7.407e+04 & 7.407e+04 & 7.406e+04 & 0.0\% & 1.9 & 2.0 & 2.6 & 9.3\\
 & 1888rte & M & 5.986e+04 & N & 5.960e+04 & 0.4\% & \dcolcolor{red} 3,\!264 & 31.6 & \dcolcolor{red} 1.1 & 14.8\\
 & 1951rte & 8.174e+04 & I & N & 8.174e+04 & 0.0\% & 20.6 & \dcolcolor{red} 61.8 & \dcolcolor{red} 1.4 & 17.6\\
 & ACTIVSg2000 & 1.228e+06 & 1.228e+06 & 1.228e+06 & 1.228e+06 & 0.0\% & 7.6 & 2.8 & 8.3 & 116\\
 & 2383wp & 1.869e+06 & 1.869e+06 & 1.869e+06 & 1.863e+06 & 0.3\% & 3.1 & 3.4 & 3.5 & 63.8\\
 & 2736sp & 1.308e+06 & 1.308e+06 & 1.308e+06 & 1.307e+06 & 0.1\% & 3.3 & 3.0 & 3.5 & 64.6\\
 & 2737sop & 7.776e+05 & 7.776e+05 & 7.776e+05 & 7.772e+05 & 0.1\% & 2.8 & 3.0 & 3.3 & 60.3\\
 & 2746wp & 1.632e+06 & 1.632e+06 & 1.632e+06 & 1.631e+06 & 0.0\% & 3.3 & 3.0 & 3.6 & 70.1\\
 & 2746wop & 1.208e+06 & 1.208e+06 & 1.208e+06 & 1.208e+06 & 0.0\% & 3.0 & 3.1 & 3.8 & 72.3\\
 & 2848rte & M & I & N & 5.301e+04 &  \textemdash  & \dcolcolor{red} 3,\!062 & \dcolcolor{red} 20.4 & \dcolcolor{red} 2.2 & 21.4\\
 & 2868rte & M & 7.979e+04 & N & 7.980e+04 & -0.0\% & \dcolcolor{red} 780 & 47.2 & \dcolcolor{red} 2.7 & 25.7\\
 & 2869pegase & 1.340e+05 & 1.340e+05 & 1.340e+05 & 1.340e+05 & 0.0\% & 3.3 & 3.3 & 5.2 & 25.9\\
 & 3012wp & 2.592e+06 & 2.592e+06 & 2.592e+06 & 2.588e+06 & 0.1\% & 4.8 & 4.8 & 5.5 & 112\\
 & 3120sp & 2.143e+06 & 2.143e+06 & 2.143e+06 & 2.141e+06 & 0.1\% & 5.1 & 4.3 & 6.2 & 122\\
 & 3375wp & 7.412e+06 & 7.412e+06 & 7.412e+06 & 7.408e+06 & 0.1\% & 8.5 & 4.6 & 8.4 & 97.6\\
 & 6468rte & 8.683e+04 & 8.683e+04 & N & 8.681e+04 & 0.0\% & 1,\!530 & 93.9 & \dcolcolor{red} 12.3 & 83.5\\
 & 6470rte & M & I & N & 9.834e+04 &  \textemdash  & \dcolcolor{red} 53.4 & \dcolcolor{red} 18.3 & \dcolcolor{red} 24.6 & 101\\
 & 6495rte & M & I & N & 1.061e+05 &  \textemdash  & \dcolcolor{red} 2,\!943 & \dcolcolor{red} 124 & \dcolcolor{red} 10.5 & 104\\
 & 6515rte & 1.098e+05 & 1.098e+05 & N & 1.097e+05 & 0.1\% & 1,\!060 & 108 & \dcolcolor{red} 12.4 & 106\\
 & 9241pegase & 3.159e+05 & 3.159e+05 & 3.159e+05 & 3.159e+05 & 0.0\% & 70.9 & 100 & 24.0 & 183\\
 & ACTIVSg10k & 2.486e+06 & I & N & 2.486e+06 & -0.0\% & 74.3 & \dcolcolor{red} 139 & \dcolcolor{red} 58.3 & 351\\
 & 13659pegase & M & 3.861e+05 & N & 3.861e+05 & -0.0\% & \dcolcolor{red} 125 & 171 & \dcolcolor{red} 4,\!925 & 145\\
 & ACTIVSg25k & 6.018e+06 & 6.018e+06 & N & 6.016e+06 & 0.0\% & 91.0 & 64.8 & \dcolcolor{red} 103 & 3,\!592\\
\hline
\iffalse
\multirow{19}{*}{\rotatebox[origin=c]{90}{PGLIB}}
 & 1354\_pegase & 1.364e+06 & 1.364e+06 & 1.364e+06 & 1.356e+06 & 0.6\% & 2.2 & 2.1 & 2.9 & 18.1\\
 & 1888\_rte & 1.565e+06 & I & N & 1.538e+06 & 1.8\% & 136 & \dcolcolor{red} 15.0 & \dcolcolor{red} 2.8 & 33.1\\
 & 1951\_rte & M & I & N & 2.375e+06 &  \textemdash  & \dcolcolor{red} 1,\!433 & \dcolcolor{red} 26.4 & \dcolcolor{red} 1.2 & 37.9\\
 & 2383wp\_k & 1.869e+06 & 1.869e+06 & 1.869e+06 & 1.862e+06 & 0.4\% & 3.1 & 3.6 & 3.5 & 75.0\\
 & 2736sp\_k & 1.308e+06 & 1.308e+06 & 1.308e+06 & 1.307e+06 & 0.1\% & 3.4 & 3.0 & 3.6 & 80.3\\
 & 2737sop\_k & 7.776e+05 & 7.776e+05 & 7.776e+05 & 7.773e+05 & 0.0\% & 2.8 & 2.8 & 3.5 & 73.1\\
 & 2746wop\_k & 1.208e+06 & 1.208e+06 & 1.208e+06 & 1.208e+06 & 0.1\% & 3.2 & 3.1 & 3.9 & 91.2\\
 & 2746wp\_k & 1.632e+06 & 1.632e+06 & 1.632e+06 & 1.631e+06 & 0.1\% & 3.9 & 2.9 & 5.6 & 88.9\\
 & 2848\_rte & 1.385e+06 & 1.385e+06 & N & 1.384e+06 & 0.1\% & 56.6 & 30.0 & \dcolcolor{red} 8.7 & 53.0\\
 & 2868\_rte & 2.260e+06 & 2.260e+06 & N & 2.260e+06 & 0.0\% & 24.5 & 21.3 & \dcolcolor{red} 7.9 & 56.5\\
 & 2869\_pegase & 2.605e+06 & 2.605e+06 & 2.605e+06 & 2.603e+06 & 0.1\% & 7.3 & 5.6 & 7.3 & 58.2\\
 & 3012wp\_k & 2.601e+06 & 2.601e+06 & 2.601e+06 & 2.596e+06 & 0.2\% & 5.6 & 4.2 & 13.6 & 127\\
 & 3120sp\_k & 2.146e+06 & 2.146e+06 & 2.146e+06 & 2.145e+06 & 0.0\% & 4.0 & 4.1 & 6.7 & 143\\
 & 6468\_rte & M & I & N & 2.251e+06 &  \textemdash  & \dcolcolor{red} 6,\!922 & \dcolcolor{red} 45.0 & \dcolcolor{red} 4.0 & 274\\
 & 6470\_rte & M & 2.556e+06 & N & 2.545e+06 & 0.4\% & \dcolcolor{red} 95.4 & 56.7 & \dcolcolor{red} 8.0 & 245\\
 & 6495\_rte & M & I & N & 2.966e+06 &  \textemdash  & \dcolcolor{red} 7,\!139 & \dcolcolor{red} 32.7 & \dcolcolor{red} 8.9 & 256\\
 & 6515\_rte & N & I & N & 2.991e+06 &  \textemdash  & \dcolcolor{red} 31,\!788 & \dcolcolor{red} 243 & \dcolcolor{red} 19.8 & 270\\
 & 9241\_pegase & 6.775e+06 & 6.775e+06 & N & 6.770e+06 & 0.1\% & 190 & 45.8 & \dcolcolor{red} 75.2 & 525\\
 & 13659\_pegase & 1.078e+07 & 1.078e+07 & 1.078e+07 & 1.078e+07 & 0.0\% & 96.4 & 70.1 & 78.4 & 563\\
\hline
\multirow{19}{*}{\rotatebox[origin=c]{90}{PGLIB SAD}}
 & 1354\_pegase & 1.365e+06 & 1.365e+06 & 1.365e+06 & 1.356e+06 & 0.6\% & 2.6 & 2.3 & 3.1 & 18.0\\
 & 1888\_rte & M & I & N & 1.538e+06 &  \textemdash  & \dcolcolor{red} 511 & \dcolcolor{red} 38.2 & \dcolcolor{red} 8.7 & 32.1\\
 & 1951\_rte & 2.382e+06 & 2.382e+06 & N & 2.376e+06 & 0.3\% & 16.8 & 30.2 & \dcolcolor{red} 1.2 & 35.7\\
 & 2383wp\_k & 1.916e+06 & 1.916e+06 & 1.916e+06 & 1.907e+06 & 0.5\% & 3.6 & 3.8 & 3.8 & 73.7\\
 & 2736sp\_k & 1.329e+06 & 1.329e+06 & 1.329e+06 & 1.324e+06 & 0.4\% & 4.2 & 3.8 & 4.6 & 77.6\\
 & 2737sop\_k & 7.927e+05 & 7.927e+05 & 7.927e+05 & 7.852e+05 & 0.9\% & 4.3 & 3.9 & 4.5 & 81.1\\
 & 2746wp\_k & 1.667e+06 & 1.667e+06 & 1.667e+06 & 1.661e+06 & 0.4\% & 4.2 & 3.8 & 4.5 & 90.1\\
 & 2746wop\_k & 1.234e+06 & 1.234e+06 & 1.234e+06 & 1.225e+06 & 0.8\% & 4.1 & 3.5 & 4.4 & 96.1\\
 & 2848\_rte & M & 1.388e+06 & N & 1.385e+06 & 0.2\% & \dcolcolor{red} 69.0 & 59.4 & \dcolcolor{red} 3.7 & 52.9\\
 & 2868\_rte & M & 2.271e+06 & N & 2.263e+06 & 0.3\% & \dcolcolor{red} 4,\!542 & 99.9 & \dcolcolor{red} 3.0 & 58.7\\
 & 2869\_pegase & 2.620e+06 & 2.620e+06 & 2.620e+06 & 2.616e+06 & 0.2\% & 11.4 & 21.3 & 8.9 & 53.7\\
 & 3012wp\_k & 2.621e+06 & 2.621e+06 & 2.621e+06 & 2.609e+06 & 0.5\% & 7.5 & 6.8 & 26.9 & 129\\
 & 3120sp\_k & 2.176e+06 & 2.176e+06 & 2.176e+06 & 2.163e+06 & 0.6\% & 5.4 & 5.6 & 7.0 & 146\\
 & 6468\_rte & M & I & N & 2.251e+06 &  \textemdash  & \dcolcolor{red} 5,\!251 & \dcolcolor{red} 38.4 & \dcolcolor{red} 3.9 & 315\\
 & 6470\_rte & M & I & N & 2.547e+06 &  \textemdash  & \dcolcolor{red} 4,\!649 & \dcolcolor{red} 828 & \dcolcolor{red} 57.4 & 239\\
 & 6495\_rte & M & I & N & 2.966e+06 &  \textemdash  & \dcolcolor{red} 48,\!228 & \dcolcolor{red} 52.4 & \dcolcolor{red} 43.1 & 258\\
 & 6515\_rte & M & I & N & 2.992e+06 &  \textemdash  & \dcolcolor{red} 68,\!374 & \dcolcolor{red} 147 & \dcolcolor{red} 19.1 & 265\\
 & 9241\_pegase & 6.917e+06 & 6.917e+06 & N & 6.821e+06 & 1.4\% & 167 & 33.3 & \dcolcolor{red} 37.5 & 549\\
 & 13659\_pegase & 1.090e+07 & 1.090e+07 & 1.090e+07 & 1.082e+07 & 0.7\% & 77.1 & 107 & 60.3 & 617\\
\hline
\multirow{12}{*}{\rotatebox[origin=c]{90}{PGLIB API}}
 & 1888\_rte & M & I & N & 2.249e+06 &  \textemdash  & \dcolcolor{red} 3,\!952 & \dcolcolor{red} 21.9 & \dcolcolor{red} 3.0 & 35.2\\
 & 2383wp\_k & 2.791e+05 & 2.791e+05 & 2.791e+05 & 2.790e+05 & 0.0\% & 1.8 & 1.6 & 2.1 & 61.4\\
 & 2736sp\_k & 6.385e+05 & 6.385e+05 & 6.385e+05 & 6.211e+05 & 2.7\% & 3.7 & 4.1 & 4.2 & 81.0\\
 & 2737sop\_k & 4.028e+05 & 4.028e+05 & 4.028e+05 & 3.985e+05 & 1.1\% & 3.9 & 3.7 & 3.9 & 56.7\\
 & 2746wop\_k & 5.117e+05 & 5.117e+05 & 5.117e+05 & 5.115e+05 & 0.0\% & 1.8 & 2.1 & 2.0 & 71.7\\
 & 2746wp\_k & 5.818e+05 & 5.818e+05 & 5.818e+05 & 5.814e+05 & 0.1\% & 2.0 & 2.4 & 2.5 & 67.4\\
 & 3012wp\_k & 7.289e+05 & 7.289e+05 & 7.289e+05 & 7.285e+05 & 0.0\% & 2.9 & 2.8 & 21.4 & 98.1\\
 & 3120sp\_k & N & 9.203e+05 & 9.203e+05 & 8.194e+05 & 11.0\% & \dcolcolor{red} 15.4 & 5.6 & 6.8 & 137\\
 & 6468\_rte & 2.710e+06 & I & N & 2.710e+06 & 0.0\% & 37,\!272 & \dcolcolor{red} 43.8 & \dcolcolor{red} 9.2 & 306\\
 & 6470\_rte & M & 3.160e+06 & N & 3.156e+06 & 0.1\% & \dcolcolor{red} 24,\!466 & 189 & \dcolcolor{red} 11.7 & 226\\
 & 6495\_rte & M & I & N & 3.576e+06 &  \textemdash  & \dcolcolor{red} 67,\!309 & \dcolcolor{red} 229 & \dcolcolor{red} 3.6 & 250\\
 & 6515\_rte & M & I & N & 3.534e+06 &  \textemdash  & \dcolcolor{red} 99,\!165 & \dcolcolor{red} 140 & \dcolcolor{red} 6.7 & 257\\
\fi
\hline
\end{tabular}
%\end{minipage}
\end{sidewaystable}
